AFSI: Automated Fluid-Structure Interaction Solver Development for Nonlinear Solid Mechanics

AFSI is a novel, open-source fluid-structure interaction (FSI) solver that extends the capabilities of the FEniCS finite element library through an immersed boundary (IB) framework. Designed to simulate large deformations in hyperelastic materials (such as cardiac tissue), AFSI avoids the need for expensive remeshing by coupling a Lagrangian representation of the solid with an Eulerian description of the surrounding fluid. This approach retains the full expressiveness of FEniCS's variational formulations, function spaces, and time integration schemes. Implemented in a hybrid Python/C++ architecture, AFSI allows users to define geometries, constitutive models (e.g., the Holzapfel-Ogden law for myocardium), and strain energy functions directly in Python, while delegating performance-critical tasks such as assembly and linear solvers to optimized C++ backends. Its concise and modular Python API facilitates the setup of FSI simulations, enabling users to easily modify discretization strategies or analyze results using standard FEniCS post-processing tools. By combining the flexibility of FEniCS with a robust immersed boundary formulation, AFSI empowers rapid prototyping of complex nonlinear solid-fluid interaction problems, making it a powerful tool for simulating biomechanical systems and other applications involving highly deformable structures in flow.

==> benchmarks/aortic-valve.tex <==

\subsection{Aortic valve model }





The AV is a thin, flexible structure located between the LV and the aorta, 
playing a crucial role in regulating blood ejection from the LV into the 
aorta during ventricular systole. 
It also ensures effective closure during diastole to prevent retrograde flow, 
thereby maintaining the unidirectional circulation of the cardiovascular system. 
This section further examines the physiological characteristics and functional mechanisms of the AV.
The AV consists of three crescent-shaped leaflets, each attached at its base to the vessel wall. 
The basal attachment points of adjacent leaflets converge to form a fibrous structure known as the 
"annulus". 
The posterior aspect of each leaflet interfaces with the aortic wall, which bulges outward to form the aortic sinus.
% In our simulation, the AV model is embedded in a rigid cylindrical tube, as done in many other studies.

The mechanical properties of the AV leaflets exhibit significant anisotropy, incompressibility, 
hyperelasticity, and nonlinearity, enabling them to undergo large deformations under physiological 
loading while maintaining functional stability. To accurately capture these mechanical behaviors, 
the FRH2 material model defined in \eqref{eq::FRH2::constitutive} is employed.
The AV model used in this subsection is based on the geometric structure of a porcine heart valve 
\cite{cai2021comparison, zhu2017vitro, flamini2016immersed}. In this model, 
the leaflet thickness is set to $0.04~\text{cm}$, and the leaflets are enclosed within a rigid 
cylindrical tube with a length of $14~\text{cm}$, wall thickness of $0.15~\text{cm}$, and an inner radius of $1.3~\text{cm}$. 
\figref{fig::aortic_valve::model::1} presents the complete FSI model, 
while \figref{fig::aortic_valve::model::fiber} illustrates the fiber distribution characteristics of the AV leaflets.
In the numerical simulation, the solid domain is discretized into $233,\!216$ tetrahedral elements with $77,\!530$ mesh nodes, 
and $465,\!797$ nodes for basis finite element function. 
The fluid domain is discretized using a structured Cartesian grid consisting of $96\times96\times192$ elements. 
The relevant physical and numerical parameters are summarized in Table~\ref{tab::aortic::valve::params}.


\begin{figure}[!ht]
    \centering
    \includegraphics[width=1.0\textwidth]{figure/aortic_valve.png}
    \caption{
        Setup of the AV model in the IB framework: the gray region represents the fixed computational domain $\Omega$, while the red region corresponds to the deformable AV.}
    \label{fig::aortic_valve::model::1}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.3\textwidth]{figure/aortic_fiber.jpg}
    \caption{
        Fiber distribution in the AV model: blue arrows denote the fiber orientation, while the red areas represent the AV leaflets.}
    \label{fig::aortic_valve::model::fiber}
\end{figure}


\begin{table}[!h]
    \centering
    \begin{tabular}{l|c|c}
        \toprule
        \textbf{Symbol} & \textbf{Value} & \textbf{Unit}  \\
        \midrule
        $\rho$  & 1.0   & $\frac{\text{g}}{\text{ml}}$ \\
        $T$ & 1.635    & $\text{s}$  \\
        $\mu$   & 4  & $\text{cP}$\\
        \midrule
        $C_{10}$  & 1210  & $\text{Pa}$\\
        $C_{01}$  & 7.99 & - \\
        $a_{f}$  & 24230 & $\text{Pa}$ \\
        $b_{f}$  & 57.62 & -    \\
        $\kappa_\text{s}$ &  $10^6$ & - \\
        \bottomrule
    \end{tabular}
    \caption{Parameters for the AV model.}
    \label{tab::aortic::valve::params}
\end{table}

For this problem, the right end of the outer tube is designated as the inlet, corresponding to the LV, while the left end is the outlet, corresponding to the aorta. The relevant boundary conditions are as follows:
\begin{itemize}
    \item   The physiological pressure of the LV is applied at the inlet of the fluid region to drive blood flow through the AV, 
            with the pressure profile over one cardiac cycle shown in \figref{fig::aortic_valve::inlet pressure}.
    \item   The outlet of the fluid region uses a three-element Windkessel model to apply dynamic pressure loading, as shown in 
            \figref{fig::aortic_valve::windkessel}. The parameters of the Windkessel model include 
            characteristic resistance $R_{c} = 0.033~\text{mmHg}\cdot\text{ml}^{-1}\cdot\text{s}$, peripheral resistance 
            $R_{p} = 0.79~\text{mmHg}\cdot\text{ml}^{-1}\cdot\text{s}$, arterial compliance $C = 1.75~\text{ml}\cdot\text{mmHg}^{-1}$, 
            with an initial pressure of $P_{Wk} = 85~\text{mmHg}$, and $P_{Ao} = P_{Wk}$, while the outlet pressure is set to $0$. 
            These parameters are referenced from \cite{cai2021comparison, stergiopulos1999total}.
    \item   Zero pressure boundary conditions are applied to the remaining boundaries of the fluid region.
\end{itemize}
\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{figure/aortic_LV_pressure.png}
        \subcaption{Left ventricular pressure profile at the inlet. }
        \label{fig::aortic_valve::inlet pressure}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figure/aortic_windkessel.png}
        \subcaption{Windkessel model at the outlet}
        \label{fig::aortic_valve::windkessel}
    \end{minipage}
    \caption{Boundary conditions applied within the AV IB framework. }
\end{figure}

The numerical simulation of the AV model encompasses two complete cardiac cycles. 
\figref{fig::aortic_valve::leaflets::deformation} presents the dynamic deformation of the valve leaflets, as computed 
using the algorithm proposed in this study. 
Figs.\,\ref{fig::aortic_valve::leaflets::deformation::sub1} and \ref{fig::aortic_valve::leaflets::deformation::sub2} 
illustrate the leaflet motion during the valve opening phase, 
whereas Figs.\,\ref{fig::aortic_valve::leaflets::deformation::sub3}, \ref{fig::aortic_valve::leaflets::deformation::sub4}, 
and \ref{fig::aortic_valve::leaflets::deformation::sub5} depict the leaflet motion during the valve closure phase.
\figref{fig::aortic_valve::streamlines} presents the velocity streamlines and pressure distributions at different time instances.
During the valve opening phase, Figs.\,\ref{fig::aortic_valve::streamlines::velocity::1}  and \ref{fig::aortic_valve::streamlines::velocity::2} illustrate the fluid flow from the LV
into the aorta. When the valve is fully open, a pronounced high-velocity jet forms, with a maximum speed of approximately $250~\text{cm}/\text{s}$.
Figs.\,\ref{fig::aortic_valve::streamlines::pressure::1} and \ref{fig::aortic_valve::streamlines::pressure::2} further show the pressure distribution, where the 
inlet pressure on the right side is slightly higher than the outlet pressure on the left, thereby 
driving the transvalvular flow. 
% During the early stage of valve closure, retrograde flow from the aorta (outlet) to the LV (inlet) is observed. 
% This reverse flow is driven by a slight pressure elevation at the outlet relative to the inlet.
Fig.\,\ref{fig::aortic_valve::streamlines::velocity::4} depict low-velocity 
fluid motion within the vessel during this phase, while Fig.\,\ref{fig::aortic_valve::streamlines::pressure::4} 
reveal a pronounced transvalvular pressure gradient across the valve leaflets. 
These observations collectively highlight the dynamic FSI characteristics inherent to the valve closure process.

\begin{figure}[htbp]
    \centering
    % 第一行
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/AV_0.12.jpg}
        \caption{0.12~\text{s}}
        \label{fig::aortic_valve::leaflets::deformation::sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/AV_0.18.jpg}
        \caption{0.18~\text{s}}
        \label{fig::aortic_valve::leaflets::deformation::sub2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/AV_0.36.jpg}
        \caption{0.36~\text{s}}
        \label{fig::aortic_valve::leaflets::deformation::sub3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/AV_0.39.jpg}
        \caption{0.39~\text{s}}
        \label{fig::aortic_valve::leaflets::deformation::sub4}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/AV_0.47.jpg}
        \caption{0.47~\text{s}}
        \label{fig::aortic_valve::leaflets::deformation::sub5}
    \end{subfigure}
    \caption{Dynamic deformation of the valve leaflets in the AV model at different time.}
    \label{fig::aortic_valve::leaflets::deformation}
\end{figure}
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[height=0.42\textwidth]{figure/AV_0.12-stream.png}
        \caption{0.12~\text{s}}
        \label{fig::aortic_valve::streamlines::velocity::1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[height=0.48\textwidth]{figure/AV_0.12-p.png}
        \caption{0.12~\text{s}}
        \label{fig::aortic_valve::streamlines::pressure::1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[height=0.42\textwidth]{figure/AV_0.18-stream.png}
        \caption{0.18~\text{s}}
        \label{fig::aortic_valve::streamlines::velocity::2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[height=0.48\textwidth]{figure/AV_0.18-p.png}
        \caption{0.18~\text{s}}
        \label{fig::aortic_valve::streamlines::pressure::2}
    \end{subfigure}
    \hfill
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[height=0.42\textwidth]{figure/AV_0.36-stream.png}
    %     \caption{0.36~\text{s}}
    %     \label{fig::aortic_valve::streamlines::velocity::3}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[height=0.48\textwidth]{figure/AV_0.36-p.png}
    %     \caption{0.36~\text{s}}
    %     \label{fig::aortic_valve::streamlines::pressure::3}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[height=0.42\textwidth]{figure/AV_0.39-stream.png}
        \caption{0.39~\text{s}}
        \label{fig::aortic_valve::streamlines::velocity::4}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[height=0.48\textwidth]{figure/AV_0.39-p.png}
        \caption{0.39~\text{s}}
        \label{fig::aortic_valve::streamlines::pressure::4}
    \end{subfigure}
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[height=0.42\textwidth]{figure/AV_0.47-stream.png}
    %     \caption{0.47~\text{s}}
    %     \label{fig::aortic_valve::streamlines::velocity::5}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.45\textwidth}
    %     \centering
    %     \includegraphics[height=0.48\textwidth]{figure/AV_0.47-p.png}
    %     \caption{0.47~\text{s}}
    %     \label{fig::aortic_valve::streamlines::pressure::5}
    % \end{subfigure}
    \caption{
        AV model velocity streamlines and pressure distribution. Left: 
        (a), (c), (e) show the velocity streamlines at $0.12~\text{s}$, $0.18~\text{s}$, 
        and  $0.39~\text{s}$ respectively. Right: (b), (d), (f) show the pressure 
        distribution at corresponding time.\label{fig::aortic_valve::streamlines}
    }
\end{figure}

\figref{fig::aortic_valve::model::flow_rate} illustrates the time-dependent variation of the flow rate for 
the AV model over the entire simulation cycle. The results show that the flow rate profile computed using the 
algorithm proposed in this study exhibits excellent agreement with the reference data reported 
in \cite{cai2021comparison}. Furthermore, the average relative error of the flow rate is
quantitatively assessed using the following equation \cite{lu2024gpu}:
\begin{align}\label{relative_errors}
    \epsilon = \frac{1}{N}\sum_{i=1}^{N} \left| \frac{Q^{\mathrm{GPU}}_{i} - Q^{\mathrm{ref}}_{i}}{\max(Q^{\mathrm{ref}}_{j})} \right| \times 100\%,
\end{align}
where $N=100$ represents the number of sampling points. $Q^{\mathrm{GPU}}$ denotes the flow rate calculated 
by  our algorithm, while $Q^{\mathrm{ref}}$ corresponds to the reference data from \cite{cai2021comparison}. Compared to the data presented in \cite{cai2021comparison}, 
the average relative error is $3.53\%$, further validating the accuracy of the proposed algorithm.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.6\textwidth]{figure/AV_flowrate.png}
    \caption{AV model flow rate diagram.}
    \label{fig::aortic_valve::model::flow_rate}
\end{figure}
\begin{table}[!h]
    \centering
    \begin{tabular}{l|l|c|c|c}
        \toprule
        \textbf{parallel scheme} & \textbf{Device} & \textbf{Number of elements} &\textbf{Time cost(s)} &\textbf{Speed-up ratio} \\
        \midrule
        GPU(Present)  & RTX4090  &  233,216  &17000   &101.02  \\
        GPU(Present)  & P100     &  233,216  &29000   &59.22  \\
        GPU(Present)  & V100     &  233,216    &27000   &63.61   \\
        CPU(IBAMR)\cite{griffith2017ibamr} & Xeon 5115($\times$2)& 196,029   &1717404   & 1.00  \\
        \bottomrule
    \end{tabular}                                                                       
    \caption{Total computational cost of the AV model on different parallel computing platforms.}
    \label{tab::aortic_valve::model::parallel}
\end{table}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.6\textwidth]{figure/AV_Time.png}
    \caption{Execution time distribution of the major algorithmic modules in the AV model across various GPU devices.}
    \label{fig::aortic_valve::model::percentage}
\end{figure}

Table \ref{tab::aortic_valve::model::parallel} summarizes the computational performance of the 
proposed algorithm for the AV model across different parallel computing platforms, including the 
GeForce RTX 4090, Tesla P100, NVIDIA V100, and dual Xeon 5112 CPUs. The speedup is defined as the 
ratio of the computation time on each platform to that of the 20-core CPU implementation based on 
the IBAMR framework, as reported in \cite{griffith2017ibamr}. The results show that the RTX 4090 
achieves a speedup of approximately $101.02\times$, while the V100 and P100 achieve about $63.61\times$ and 
$59.22\times$, respectively. 
These findings not only demonstrate the high computational efficiency 
of the proposed algorithm but also emphasize its broad compatibility across different GPUs.
In addition, \figref{fig::aortic_valve::model::percentage} presents the distribution of execution 
time among the major algorithmic 
modules across various GPU devices. The results show that the Poisson equation solver consistently 
dominates the computational cost, accounting for more than $58\%$ of the total runtime on all devices. 
The Helmholtz equation solver is the second most time-consuming component, contributing over $13\%$, 
while all other modules consume less than $10\%$ of the total time. These findings further validate 
the efficiency of the proposed algorithm and underscore its potential for targeted optimization of 
dominant computational bottlenecks.



==> benchmarks/bonet-torsion.tex <==


\subsection{Bonet's torsion problem}


主要参考：
\cite{wells2023nodal}
间接参考：
\cite{bonet2015computational}
\cite{vadala2020stabilization}




This benchmark is based on a similar test by Bonet et al. [19] and then modified by Vadala-Roth et al. [36] for an FSI framework. It involves applying torsion to the top face of an elastic beam, while the opposite face is fixed in place; see Fig. 10. Zero traction boundary conditions are applied along all other faces. The computational domain is $\Omega=[0, L]^3$ with $L=9 \mathrm{~cm}$. The Cartesian grid uses $N=\operatorname{ceil}\left(M E_{\mathrm{FAC}} M_{\mathrm{FAC}} \cdot \frac{9}{6}\right)$ cells in each coordinate direction, in which $M$ is the number of elements per edge in the Lagrangian mesh, 9 is the length of the computational domain, and 6 is the length of the structure. The time step size is $\Delta t=0.001 \Delta x s$. The structure is an elastic beam with an incompressible modified Mooney-Rivlin material model.

The torsion is imposed via displacement boundary conditions, and this face is rotated by $\theta_{\mathrm{f}}=2.5 \pi$. The material and numerical parameters are listed in Table 6. A body damping parameter of $\eta_{\mathrm{B}}=0.2 \cdot\left(c_1+c_2\right)=3600 \frac{\mathrm{~g}}{\mathrm{~cm}^3 . \mathrm{s}}$ was applied on the interior of the structural domain to dampen oscillations as the structure reaches steady state. The penalty parameter used to fix the stationary face in place is $\kappa_{\mathrm{S}}=1.25 \cdot \frac{\Delta x}{\Delta t} \frac{\mathrm{dyn}}{\mathrm{cm}^3}$. We gradually apply the traction to the solid boundary linearly in time so that the full load is applied at $T_1=2.0 \mathrm{~s}$, and we wait until time $T_{\mathrm{f}}=5.0 \mathrm{~s}$ for the structure to reach equilibrium. The number of solid DoFs range from $m=65$ to $m=12,337$. Results are presented, only for $M_{\mathrm{FAC}}=1.0$, in Figs. 11 and 12 .

Because of the greater computational costs of three-dimensional simulations, cases with finer Cartesian grids were omitted. Using the intuition of the previous benchmark results and the results of Vadala-Roth et al. [36], which show that $M_{\mathrm{FAC}}=2.0$ yields convergent results with the standard IFED method, we expect the new methods with $M_{\mathrm{FAC}}=1.0$ will converge to the benchmark solution. Indeed, this appears to be the case, as seen in Fig. 12, although more structural DoFs are needed. Fig. 12 shows that results from the elementally and nodally coupled methods are in close agreement, with the exception of $\mathcal{P}^2$ elements. Here, the $\mathcal{P}^2$ elementally coupled case encountered severe time-step restrictions resulting from the mesh factor ratio. For this reason, results for elemental coupling with $\mathcal{P}^2$ elements were omitted. However, the nodally coupled method with $\mathcal{P}^2$ elements had no such time-step restrictions, and in fact, converges to the benchmark solution offered by the FE method. In fact, this $\mathcal{P}^2$ case demonstrates faster convergence to the FE solution than the other cases shown here. Fig. 11 compares the deformations for $\mathcal{Q}^1$ elements, again indicating close qualitative agreement between deformations computed by the two methods.

==> benchmarks/cook-membrane.tex <==
% \subsection{Cook's Membrane Benchmark}

The Cook's membrane problem is a classical benchmark in incompressible elastic solid mechanics. 
To assess the computational accuracy of the fully GPU-accelerated, matrix-free IB algorithm, 
we adopt the setup described in \cite{vadala2020stabilization}, wherein the three-dimensional 
anisotropic Cook's membrane is embedded into incompressible Newtonian fluid, 
forming an FSI system that is subsequently solved numerically using the proposed method.
The configuration of the computational domain $\Omega$, structural domain, and loading conditions is shown in 
Fig.\,\ref{fig::cook_membrane::anisotropic::3}.

\begin{figure}[!ht]
\centering
\includegraphics[width=0.46\textwidth]{figure/cook3_dimension.png}
\caption{
    Setup of the anisotropic Cook's membrane benchmark: The gray region represents the fixed computational 
    domain $\Omega$, while the red region corresponds to the deformable structure.
    \label{fig::cook_membrane::anisotropic::3}
}
\end{figure}
The boundary conditions for this problem consist of a fixed left face, where constraints are enforced using 
a penalty term with a parameter of $\kappa = 10^6$. 
A vertical traction of $6.25~\frac{\text{dyn}}{\text{cm}^{2}}$ is applied to the right face, increasing gradually 
according to the polynomial function $q(t)=-2(\frac{t}{T1})^{3}+3(\frac{t}{T1})^{2}$ and reaching its maximum at 
time $T_1$, staying constant until time $T_f$.
The simulation continues until time $T_f$ to ensure the system reaches equilibrium. All other faces are subject to zero traction conditions. 
A summary of the relevant physical and numerical parameters is provided in Table \ref{tab::cook::membrane::params}.
\begin{table}[!h]
    \centering
    \begin{tabular}{l|c|c}
        \toprule
        \textbf{Symbol} & \textbf{Value} & \textbf{Unit}  \\
        \midrule
        $\rho$  & 1.0   & $\frac{\text{g}}{\text{cm}^3}$ \\
        \(T_1\) & 14    & $\text{s}$ \\
        \(T_f\) & 35    & $\text{s}$  \\
        $\mu$   & 0.16  & $\frac{\text{dyn}\cdot \text{s}}{\text{cm}^{2}}$\\
        \midrule
        $G_T$  & 8.0  & $\frac{\text{dyn}}{\text{cm}^2}$\\
        $G_L$  & 160.0 & $\frac{\text{dyn}}{\text{cm}^2}$ \\
        $E_L$  & 1200.0 & $\frac{\text{dyn}}{\text{cm}^2}$ \\
        % $\nu_{stab}$ & 0.4 &  -\\
        $\kappa_\text{stab}$ &  112 & $\frac{\text{dyn}}{\text{cm}^2}$ \\
        $\mathbf{e}_{f}$ & $\frac{1}{\sqrt{3}}(1,1,1)$ &-\\
        \bottomrule
    \end{tabular}
    \caption{Parameters for the anisotropic Cook's membrane benchmark}
    \label{tab::cook::membrane::params}
\end{table}

In this case, the computational domain $\Omega$ is discretized using a Cartesian grid 
with $N = 64$ cells along each coordinate axis. The structure is discretized using a 
tetrahedral mesh, and both forces and displacements are approximated using 
nodal finite element basis functions, as described previously. The number of structural DoFs 
ranges from $M = 5,\!004$ to $M = 282,\!489$, depending on the mesh resolution. The time step used 
in the simulation is $\Delta t = 0.001~\text{s}$.

To verify the accuracy of our computational results, we primarily focus on the deformation 
of Cook's membrane, the determinant of the deformation gradient $J$, 
and the vertical displacement at the upper-right corner, $A = (7.06~\text{cm}, 8.0~\text{cm}, 4.5~\text{cm})$, of the membrane.  
\figref{fig::cook_membrane::anisotropic::deformation} illustrates the deformation of Cook's membrane at the final time from different angles. 
The results appear to be consistent with those reported in \cite{vadala2020stabilization}.  
\figref{fig::cook_membrane::anisotropic::Jacobian} presents the computational results for $J$. Upon examining the figure, 
it is evident that $J$ remains uniformly close to $1$ throughout the entire solid.  
\figref{fig::cook_membrane::anisotropic::volume_change} 
compares the volume change percentage of Cook's membrane for various degrees of freedom with the results reported in \cite{vadala2020stabilization}. 
The analysis reveals that the volume change percentage of our results range from $0.00062\%$ to $0.0088\%$, 
closely aligning with the data presented in \cite{vadala2020stabilization}.  
Notably, the results obtained using $P2$ elements in our study are nearly identical to those calculated using $Q1$ elements.  
\figref{fig::Cook's membrane::displacement} illustrates the variation in the displacement of point $A$ along the $y$-axis over time.  
\figref{fig::Cook's membrane::displacement::nodes} shows the variation in the maximum displacement of point $A$ along the $y$-axis with different DoFs.  
Furthermore, \figref{fig::Cook's membrane::displacement::nodes} demonstrates that the displacement of point $A$ along the $y$-axis, as calculated by our method, is essentially consistent with the results reported in \cite{vadala2020stabilization}.  
This classical benchmark case clearly demonstrates the properties of our algorithm in terms of high accuracy, stability, and excellent volume conservation.


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figure/cook_membrane_deformation.png}
    \caption{Deformations of the anisotropic Cook's membrane from different angles.}
    \label{fig::cook_membrane::anisotropic::deformation}
\end{figure}

\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[height=0.6\textwidth]{figure/cook_membrane_J.png}
        \subcaption{Determinant of deformation gradient.}
        \label{fig::cook_membrane::anisotropic::Jacobian}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[height=0.6\textwidth]{figure/cook_volume_change.png}
        \subcaption{Volume change under different numbers of DoFs.}
        \label{fig::cook_membrane::anisotropic::volume_change}
    \end{minipage}
    \caption{Volume conservation for the anisotropic Cook's membrane.}
\end{figure}
\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/cook_membrane_displacement1.png}
        \subcaption{Displacement over time for a mesh with $282,\!489$ DoFs.}
        \label{fig::Cook's membrane::displacement}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/cook_membrane_displacement2.png}
        \subcaption{Displacement under different numbers of DoFs at $t=T_f$.}
        \label{fig::Cook's membrane::displacement::nodes}
    \end{minipage}
    \caption{The $y$-displacement of corner point A for the anisotropic Cook's membrane.  }
\end{figure}

% \begin{table}[!h]
%     \centering
%     \begin{tabular}{lcc|cc}
%         \toprule
%         & \multicolumn{2}{c|}{\textbf{CPU-GPU Heterogeneous}} & \multicolumn{2}{c}{\textbf{Full GPU (Present)}} \\
%         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%         & (\%) & (s) & (\%) & (s) \\
%         \midrule
%         Fluid Solver (Poisson equation) & 71.35 & 10827.8 & 72.4 & 659 \\
%         Fluid Solver (Helmholtz equation) & 26.99 & 4095.58 & 13.41 & 122 \\
%         Fluid Solver (Convective Term) & 0.34 & 51.59 & 0.15 & 1.339 \\
%         Interpolation & 1.25 & 189.31 & 0.42 & 3.804 \\
%         Spreading & 1.25 & 189.31 & 0.44 & 3.959 \\
%         Solid Solver & 1.25 & 189.31 & 8.68 & 79 \\ 
%         \bottomrule
%     \end{tabular}
%     \caption{Execution time distribution of major algorithmic modules in the anisotropic Cook's membrane model under different parallelization strategies (CPU-GPU heterogeneous vs. fully GPU-parallel)}
%     \label{tab::cook::membrane::solver}
% \end{table}

% \begin{table}[!h]
%     \centering
%     \begin{tabular}{l|c|c|c}
%         \toprule
%         \textbf{Solid Dof} & \textbf{CPU-GPU Heterogeneous(s)} & \textbf{Full GPU (Present) (s)} & \textbf{Speedup} \\
%         \midrule
%         5004   &     & 910   &  \\
%         23991  &     & 904   &  \\
%         70161  &     & 910   &  \\
%         154374 &     & 1003  &  \\
%         282489 &     & 1017  &  \\
%         \bottomrule
%     \end{tabular}
%     \caption{Full GPU parallel vs. CPU-GPU Interaction parallel: speedup comparison for different solid DoFs in solving the anisotropic Cook's membrane model.}
%     \label{tab::cook::membrane::Dof}
% \end{table}


==> benchmarks/dynamic-left-ventricle.tex <==
\subsection{Dynamic left ventricle model }

As one of the four chambers of the heart, the LV plays a crucial role in the heart's pumping function. 
This section builds upon a previously developed image-based geometric model \cite{gao2017changes}, 
similar to those used in several studies \cite{gao2014quasi, gao2014dynamic, cai2015multi}, 
and focuses on a simplified cardiac mechanics problem relevant to physiological conditions during systole and diastole. 
For this investigation, only a portion of the LV is considered (see \figref{fig::left_ventricle::model::1}).

In the LV model shown in \figref{fig::left_ventricle::model::1}, 
zero displacements are applied in the z-axis direction and along the circumferential direction at the base, 
allowing only radial expansion within the plane. Meanwhile, a uniform pressure is applied to the endocardial surface, 
which varies according to the prescribed waveform $p_{\text{endo}}(t)$, as referenced in \cite{thekkethil2023stabilized}. 
The maximum endocardial pressures during diastole and systole are $1.067~\text{kPa}$ and $14.530~\text{kPa}$, respectively, 
as defined by the following expression:

\begin{equation*}
    p_{\text{endo}}(t) =
\begin{cases}
\frac{1.067}{0.2}t \text{ kPa}, & \text{if } t < 0.2, \\[8pt]
1.067 \text{ kPa}, & \text{if } 0.2 < t < 0.5, \\[8pt]
1.067 + 13.46 \left( 1 - \exp\left( -\frac{(t - 0.5)^2}{0.004} \right) \right) \text{ kPa}, & \text{if } 0.5 < t < 0.65, \\[8pt]
1.067 + 13.46 \left( 1 - \exp\left( -\frac{(0.8 - t)^2}{0.004} \right) \right) \text{ kPa}, & \text{if } 0.65 < t < 0.8.
\end{cases}
\end{equation*}


We model the myocardium as a nonlinear, anisotropic hyperelastic material. To account for the effect of active tension, 
the first Piola-Kirchhoff stress tensor of the myocardium is modelled as the sum of the active and passive stress:
\begin{align*}
    \mathbb{P}=\frac{\partial\Psi}{\partial\mathbb{F}}+\mathbb{P}^{a},
\end{align*} 
where the passive stress component is described using the HO model defined in \eqref{eq::HO::constitutive}, the active stress component $\mathbb{P}^{a}$ is given by:
\begin{align*}
    \mathbb{P}_{a}=T(t,I_{4f})\mathbb{F}\mathbf{e}_{f}\otimes\mathbf{e}_{f},
\end{align*}
where $\mathbf{e}_{f}$ are the fiber directions, and the scalar tension $T=T(t,I_{4f})$ is a function of time $t$ and $I_{4f}$.
Specifically, 
\begin{align*}
    T(t,I_{4f})=T_{a}(t)\left(1+4.9(\sqrt{I_{4f}}-1)\right),
\end{align*}
where $T_{a}(t)$ is the active tension, which is determined empirically. 
Based on the maximum active tension value of a healthy LV reported in \cite{gao2014dynamic}, we set its expression according to \cite{thekkethil2023stabilized}, as follows:
\begin{equation*}
    T_a(t) =
    \begin{cases} 
    0 \text{ kPa}, & \text{if } t < 0.5, \\ 
    84.26 \left( 1 - \exp \left( \frac{-(t - 0.5)^2}{0.005} \right) \right) \text{ kPa}, & \text{if } 0.5 < t < 0.65, \\ 
    84.26 \left( 1 - \exp \left( \frac{-(0.8 - t)^2}{0.005} \right) \right) \text{ kPa}, & \text{if } 0.65 < t < 0.8.
    \end{cases} 
\end{equation*}
The detailed physical and numerical parameters are listed in Table~\ref{tab::left::ventricle::params}. 
In the numerical simulation, the solid domain is discretized into $133,\!042$ tetrahedral elements with $25,\!933$ nodes for the mesh, 
and $192,\!322$ nodes used for the finite element basis functions. The fluid domain is discretized using a Cartesian grid consisting of $96 \times 96 \times 96$ grid cells.
\begin{figure}[!ht]
\centering
\includegraphics[width=0.4\textwidth]{figure/left_ventricle_model.png}
\caption{
    Setup of the LV model in the IB framework: the gray region represents the fixed computational domain $\Omega$, while the red region corresponds to the deformable LV.
}
\label{fig::left_ventricle::model::1}
\end{figure}

\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=0.55\textwidth]{figure/LV_f0.jpg}
        \subcaption{Fiber directions: $\mathbf{e}_{f}$.}
        \label{fig::left_ventricle::f0}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=0.55\textwidth]{figure/LV_s0.jpg}
        \subcaption{Sheet directions: $\mathbf{e}_{s}$.}
        \label{fig::left_ventricle::s0}
    \end{minipage}
    \caption{
        Fiber distribution in the LV model in reference configuration.}
\end{figure}


\begin{table}[!h]
    \centering
    \begin{tabular}{l|c|c}
        \toprule
        \textbf{Symbol} & \textbf{Value} & \textbf{Unit}  \\
        \midrule
        $\rho$  & 1.0   & $\frac{\text{g}}{\text{cm}^3}$ \\
        $T$ & 2.4    & $\text{s}$  \\
        $\mu$   & 0.04  & $\frac{\text{dyn}\cdot \text{s}}{\text{cm}^{2}}$\\
        \midrule
        $a$  & 2244.87  & $\frac{\text{dyn}}{\text{cm}^2}$\\
        $a_{f}$  & 24267 & $\frac{\text{dyn}}{\text{cm}^2}$ \\
        $a_{s}$  & 5562.38 & $\frac{\text{dyn}}{\text{cm}^2}$ \\
        $a_{fs}$  & 3905.16 & $\frac{\text{dyn}}{\text{cm}^2}$ \\
        $b$  & 1.6215 &  -    \\
        $b_{f}$  & 1.8268 & -    \\
        $b_{s}$  &  0.7746 & -   \\
        $b_{fs}$  & 1.695 & - \\
        $\kappa_\text{s}$ &  $5\times10^6$ & - \\
        \bottomrule
    \end{tabular}
    \caption{Parameters for the dynamic LV model.}
    \label{tab::left::ventricle::params}
\end{table}

In this model, three consecutive cardiac cycles are simulated, covering both the diastolic and systolic phases of each cycle. 
For efficiency comparison, we also ran the same model on a CPU-GPU heterogeneous computing platform, 
which is an early-stage exploratory implementation of our fully GPU-accelerated FSI solver. 
The solid mechanics solver—due to its complexity and the need to support diverse material models—was executed on the CPU, 
while the remaining components were run on the GPU. 
Given the intrinsic nature of our algorithm, frequent interactions between the solid and fluid domains were required. 
The data exchange between the CPU and GPU introduced significant overhead, 
with host-to-device and device-to-host memory transfers substantially exceeding the time required to solve equations. 
As a result, the total simulation time on the CPU-GPU platform was $129,730$ seconds, while the fully GPU-accelerated simulation completed in approximately $2,233$ seconds, achieving a speedup of 58 times, thereby validating the necessity of the fully GPU-based solver.
\figref{fig::left_ventricle::deformation} illustrates the deformation of the LV, 
with \figref{fig::left_ventricle::deformation::diastole} showing the LV during the diastolic phase 
and \figref{fig::left_ventricle::deformation::systole} depicting it during the systolic phase. 
\figref{fig::left_ventricle::slice} presents cross-sectional views of LV deformation and the 
corresponding velocity streamlines at $0.12~\text{s}$, $0.45~\text{s}$, and $0.72~\text{s}$.
As shown in \figref{fig::left_ventricle::slice}, the LV is in the diastolic phase at $0.12~\text{s}$ and $0.45~\text{s}$, 
during which blood flows into the ventricular cavity. By $0.45~\text{s}$, 
the LV is approaching its maximal diastolic expansion. The streamline pattern at this moment 
reveals a significant reduction in flow velocity, 
indicating a decrease in the inflow rate and suggesting that the cavity volume is nearing 
its peak—reflecting the physiological process of ventricular filling.
At $0.72~\text{s}$, the LV enters the systolic phase, and myocardial contraction ejects 
blood from the cavity. This is evidenced by the reversal of the streamline direction and tissue deformation along the contraction direction. 
Additionally, due to the incompressible nature of myocardial tissue, the ventricular wall thickens. 
In our results, the end-diastolic volume (EDV) and end-systolic volume (ESV) are 86.06 ml and 36.42 ml, respectively. 
The stroke volume (SV) is 49.64 ml, and the ejection fraction (EF) is 57.68\%, which falls within the normal range for a healthy individual.
These behaviors correspond to the typical physiological motion of the LV during a cardiac cycle, 
reflecting the pressure-generating effect of myocardial contraction.
\figref{fig::left_ventricle::volume1} shows the temporal evolution of the wall volume of the LV. 
Both the purely solid finite element simulation and the FSI simulation presented in this study accurately 
capture the incompressibility of the myocardial material.
% As myocardial tissue is generally regarded as incompressible under normal physiological conditions, 
% the calculated LV volume remains nearly constant throughout the cardiac cycle—consistent with predictions from a purely solid mechanics model. 
% This supports the validity of the incompressibility assumption used in the simulation. 
% In contrast, \figref{fig::left_ventricle::volume2} presents the dynamic variation of the LV cavity volume over time, 
% capturing the volumetric fluctuations associated with the filling and ejection phases. 
% These results emphasize the dynamic characteristics of left ventricular pumping function from a volumetric perspective.

\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=0.7\textwidth]{figure/LV_origin.jpg}
        \subcaption{Original position}
        \label{fig::left_ventricle::deformation::origin}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=0.65\textwidth]{figure/LV_shuzhang.jpg}
        \subcaption{Diastole}
        \label{fig::left_ventricle::deformation::diastole}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=0.60\textwidth]{figure/LV_shousuo.jpg}
        \subcaption{Systole}
        \label{fig::left_ventricle::deformation::systole}
    \end{minipage}
    \caption{Schematic illustration of left ventricular deformation. The red color indicates the deformed position, while the grey 
    color indicates the original position.}
    \label{fig::left_ventricle::deformation}
\end{figure}

\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/LV_0.12s.jpg}
        \subcaption{$0.12~\text{s}$}
        \label{fig::left_ventricle::0.12s}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/LV_0.45s.jpg}
        \subcaption{$0.45~\text{s}$}
        \label{fig::left_ventricle::0.45s}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/LV_0.72s.jpg}
        \subcaption{$0.72~\text{s}$}
        \label{fig::left_ventricle::0.72s}
    \end{minipage}
    \caption{Deformation of a left ventricular slice and fluid velocity streamlines at different times.}
    \label{fig::left_ventricle::slice}
\end{figure}

\begin{figure}[!ht]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/LV_volume.png}
        
    \end{minipage}
    % \begin{minipage}{0.45\textwidth}
    %     \centering
    %     \includegraphics[width=1.0\textwidth]{figure/LV_volume2.png}
    %     \subcaption{Capacity}
    %     \label{fig::left_ventricle::volume2}
    % \end{minipage}
    \caption{Time-dependent changes of the wall volume.\label{fig::left_ventricle::volume1}}
\end{figure}

% \begin{table}[!h]
%     \centering
%     \begin{tabular}{lcc|cc}
%         \toprule
%         & \multicolumn{2}{c|}{\textbf{CPU-GPU Heterogeneous}} & \multicolumn{2}{c}{\textbf{Full GPU (Present)}} \\
%         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%         & (\%) & (s) & (\%) & (s) \\
%         \midrule
%         Poisson equation & 71.35 & 10827.8 & 57.01 & 1273 \\
%         Helmholtz equation & 26.99 & 4095.58 & 9.85 & 220 \\
%         Convective Term & 0.34 & 51.59 & 0.08 & 1.873 \\
%         Interpolation & 1.25 & 189.31 & 1.16 & 26 \\
%         Spreading & 1.25 & 189.31 & 1.4 & 46 \\
%         Solid Solver & 1.25 & 189.31 & 25.93 & 579 \\ 
%         Total time      & & &  &  2233\\
%         \bottomrule
%     \end{tabular}
%     \caption{Execution time distribution of major algorithmic modules in the LV model under different parallelization strategies (CPU-GPU heterogeneous vs. fully GPU-parallel)}
% \end{table}



==> benchmarks/mitral-valve.tex <==

\subsection{Mitral valve model}




The MV is located between the left atrium (LA) and the LV. 
It opens during diastole to facilitate blood flow into the 
LV and closes during systole to prevent backflow into the LA.
The proper function of the MV is critical for maintaining effective blood flow out of the heart 
and minimizing the hemodynamic load on the cardiovascular system. 
This section provides a detailed examination of the MV's physiological properties and dynamic behavior. 
Compared to the AV, the MV has a more intricate structure, comprising two main valve leaflets (anterior and posterior), 
the mitral annulus, chordae tendineae, and papillary muscles. 
The valve leaflets are asymmetrical, and the mitral annulus is anchored to the left ventricular wall. 
The interaction between the valve leaflets and the annulus ensures that blood does not flow 
back into the left atrium during ventricular contraction. The chordae tendineae connect the valve leaflets 
to the papillary muscles, primarily controlling the motion of the leaflets. The papillary muscles, 
which are fixed to the left ventricular wall, act as anchor points for the chordae tendineae, 
further regulating the motion of the valve leaflets. This complex structural interaction is crucial 
for the proper function of the MV.


To accurately characterize the complex mechanical behavior of the MV leaflets—namely their pronounced anisotropy, 
incompressibility, hyperelasticity, and nonlinearity—we adopt FRH1 model, defined in \eqref{eq::FRH1::constitutive}, to describe
their constitutive response \cite{cai2019some, gao2014finite}.
The mechanical behavior of the chordae tendineae is described using a linear elastic Neo-Hookean model, 
which reasonably captures their elastic deformation characteristics under physiological conditions \cite{cai2019some, gao2014finite}. 
The strain energy function for this model is given by:
$$\Psi=a(\bar{I}_{1}-3)+\frac{\kappa_{\text{stab}}}{2}\left(\text{ln}(J)\right)^{2},$$
and its first Piola-Kirchhoff stress tensor is:
$$\mathbb{P}=2aJ^{-2/3}\left(\mathbb{F}-\frac{I_{1}}{3}\mathbf{F}^{-T}\right)+\kappa_{\text{stab}}\text{ln}({J})\mathbb{F}^{-T}.$$
This section is based on the previously developed image-based geometric model of the MV \cite{cai2019some, gao2014finite, ma2013image}. 
In the model, the thickness of the valve leaflets is set to $0.1~\text{cm}$, and the length of the surrounding rigid circular tube is $16~\text{cm}$, with a radius of $3.8~\text{cm}$. 
The complete FSI model is shown in Fig.\,\ref{fig::mitral_valve::model::origin}, and the fiber distribution within the valve leaflets is illustrated 
in Fig.\,\ref{fig::mitral_valve::model::fiber}. 
In the numerical simulations, the solid domain is discretized into 734,645 tetrahedral elements and 188,557 mesh nodes, 
with 1,245,119 nodes used for basis functions. Meanwhile, the fluid region is discretized into a Cartesian grid of $80 \times 80 \times 128$ elements. 
The relevant physical and numerical parameters are provided in Table \ref{tab::mitral::valve::params}.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figure/mitral_valve.png}
    \caption{Setup of the MV model in the IB framework: the gray region represents the fixed computational domain $\Omega$, while the red region corresponds to the deformable MV.}
    \label{fig::mitral_valve::model::origin}
\end{figure}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.3\textwidth]{figure/mitral_fiber.jpg}
    \caption{Fiber distribution in the MV model. Blue arrows indicate the direction of fibers, and red represents the MV leaflets.}
    \label{fig::mitral_valve::model::fiber}
\end{figure}
\begin{table}[!h]
    \centering
    \begin{tabular}{l|c|c|c}
        \toprule
        \textbf{Type} &\textbf{Symbol} & \textbf{Value} & \textbf{Unit}  \\
        \midrule
        -    &$\rho$  & 1.0   & $\frac{\text{g}}{\text{cm}^3}$ \\
        -    &$T$      & 2     & $\text{s}$  \\
        -    &$\mu$    & 0.04  & $\frac{\text{dyn}\cdot \text{s}}{\text{cm}^{2}}$\\
        \midrule
        Anterior leaflet    &$C_1$  & 17400  & $\text{Pa}$\\
        Anterior leaflet   &$a_{f}$  & 31300 & $\text{Pa}$ \\
        Anterior leaflet   &$b_{f}$  & 55.93 & -    \\
        -                           &$\kappa_\text{s}$ &  $10^7$ & - \\
        \midrule
        Posterior leaflet    &$C_1$  & 10200  & $\text{Pa}$\\
        Posterior leaflet   &$a_{f}$  & 50000 & $\text{Pa}$ \\
        Posterior leaflet    &$b_{f}$  & 63.48 & -    \\
        -                           &$\kappa_\text{s}$ &  $10^7$ & - \\
        \midrule
        Chordae tendineae(systole)  &   $C$   &9.0  &$\text{MPa}$ \\
        Chordae tendineae(diastole) &   $C$   &0.54  &$\text{MPa}$\\
        -                           &$\kappa_\text{s}$ &  $10^7$ & - \\      
        \bottomrule
    \end{tabular}
    \caption{Parameters for the MV model.}
    \label{tab::mitral::valve::params}
\end{table}

The boundary conditions for the FSI system of the MV model are set as follows:
\begin{itemize}
    \item A transvalvular pressure difference is defined between the inlet and outlet of the tube based on a typical human physiological pressure curve (as shown in Fig.\,\ref{fig::mitral_valve::model::pressure}).
    \item Zero-pressure boundary conditions are applied along the remainder boundaries of the fluid region \cite{gao2014finite, ma2013image}.
\end{itemize}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figure/mitral_pressure.png}
    \caption{The pressure profiles prescribed at the inlet and outlet of the tube in the MV model to define the transvalvular pressure difference.}
    \label{fig::mitral_valve::model::pressure}
\end{figure}
\begin{figure}[!ht]
    \centering
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \begin{minipage}[t]{\textwidth}
            \centering
            \includegraphics[height=0.43\textwidth]{figure/0.10.png}
            \subcaption{$0.10~\text{s}$}
            \label{fig::mitral_valve::model::velocity_and_pressure::a}
        \end{minipage}
        \vfill
        \begin{minipage}[t]{\textwidth}
            \centering
            \includegraphics[height=0.43\textwidth]{figure/0.22.png}
            \subcaption{$0.22~\text{s}$}
            \label{fig::mitral_valve::model::velocity_and_pressure::b}
        \end{minipage}
        \vfill
        \begin{minipage}[t]{\textwidth}
            \centering
            \includegraphics[height=0.43\textwidth]{figure/0.35.png}
            \subcaption{$0.35~\text{s}$}
            \label{fig::mitral_valve::model::velocity_and_pressure::c}
        \end{minipage}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \begin{minipage}[t]{\textwidth}
            \centering
            \includegraphics[height=0.43\textwidth]{figure/MV_pressure_0.10s.png}
            \subcaption{$0.10~\text{s}$}
            \label{fig::mitral_valve::model::velocity_and_pressure::d}
        \end{minipage}
        \vfill
        \begin{minipage}[t]{\textwidth}
            \centering
            \includegraphics[height=0.43\textwidth]{figure/MV_pressure_0.22s.png}
            \subcaption{$0.22~\text{s}$}
            \label{fig::mitral_valve::model::velocity_and_pressure::e}
        \end{minipage}
        \vfill
        \begin{minipage}[t]{\textwidth}
            \centering
            \includegraphics[height=0.43\textwidth]{figure/MV_pressure_0.35s.png}
            \subcaption{$0.35~\text{s}$}
            \label{fig::mitral_valve::model::velocity_and_pressure::f}
        \end{minipage}
    \end{minipage}
    \caption{MV model velocity streamlines and pressure distribution. Left: (a), (b), (c) show the velocity streamlines at $0.1~\text{s}$, $0.22~\text{s}$, and $0.35~\text{s}$, respectively. Right: (d), (e), (f) show the pressure distribution at the same time.}
    \label{fig::mitral_valve::model::velocity_and_pressure}
\end{figure}

In this MV model, the LV is excluded, and the simulation focuses solely on the rapid 
filling phase of diastole and the systolic phase. The total computational time  is set to one complete cardiac cycle, 
with a duration of $0.8~\text{s}$. 
Fig.\,\ref{fig::mitral_valve::model::velocity_and_pressure} illustrates the velocity streamlines, pressure distribution, and the deformation of the MV leaflets 
and chordae tendineae. As shown in Fig.\,\ref{fig::mitral_valve::model::velocity_and_pressure::a}, when the valve is fully open ($t = 0.1~\text{s}$), a strong jet of blood is observed flowing toward the outlet. 
Fig.\,\ref{fig::mitral_valve::model::velocity_and_pressure::d} demonstrates that the valve opens under a driving pressure difference of approximately $10~\text{mmHg}$, accompanied by significant pressure variations near the valve. 
In Fig.\,\ref{fig::mitral_valve::model::velocity_and_pressure::b}, when the valve has just closed ($t = 0.22~\text{s}$), regurgitation occurs, which is considered a primary mechanism for the first heart sound \cite{gao2014finite}. 
Fig.\,\ref{fig::mitral_valve::model::velocity_and_pressure::c} shows the velocity distribution at the peak of the transvalvular pressure gradient. 
Finally, Figs.\,\ref{fig::mitral_valve::model::velocity_and_pressure::e} and \ref{fig::mitral_valve::model::velocity_and_pressure::f} demonstrate that the valves fully close under a transvalvular pressure difference of approximately $80~\text{mmHg}$, followed by slight additional deformation as the transmembrane pressure difference increases to a peak value of $150~\text{mmHg}$.


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.6\textwidth]{figure/mitral_valve_flow_rate.png}
    \caption{MV model flow rate diagram.}
    \label{fig::mitral_valve::model::flow_rate}
\end{figure}

Fig.\,\ref{fig::mitral_valve::model::flow_rate} illustrates the temporal evolution of the flow rate over a $0.5~\text{s}$ period for the MV model and presents a comparative analysis between the results
 obtained in this study 
and the simulation data reported in \cite{cai2019some, gao2014finite}. The results indicate that the flow rate curve obtained by our method shows excellent agreement with the reference data, demonstrating strong performance in terms of both accuracy and stability.
Furthermore, the average relative error of the flow rate was quantitatively evaluated using \eqref{relative_errors}. Compared with the simulation results in \cite{cai2019some}, the average relative error is $\epsilon = 3.41\%$, 
while the comparison with \cite{gao2014finite} yields an error of $\epsilon = 4.39\%$. These findings further validate the high accuracy and reliability of the proposed algorithm in predicting flow rate.

\begin{table}[!h]
    \centering
    \begin{tabular}{l|l|c|c|c}
        \toprule
        \textbf{Parallel scheme} & \textbf{Device} & \textbf{Number of elements} &\textbf{Time cost(s)} &\textbf{Speed-up ratio} \\
        \midrule
        GPU(Present)  & RTX4090  &   734,645 &2908   & 57.28  \\
        GPU(Present)  & P100     &   734,645  &5751   &28.96 \\
        GPU(Present)      & V100     &   734,645  &4726   &35.24   \\
        CPU(IBAMR)\cite{griffith2017ibamr} & Xeon 5115($\times$2)& 260,053   &166559   & 1.00  \\
        \bottomrule
    \end{tabular}                                                                       
    \caption{Total computational cost of the MV model on different parallel computing platforms.}
    \label{tab::mitral_valve::model::parallel}
\end{table}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.6\textwidth]{figure/MV_Time.png}
    \caption{Execution time distribution of the major algorithmic modules in the MV model across various GPU devices.}
    \label{fig::mitral_valve::model::percentage}
\end{figure}

To evaluate the computational efficiency of the proposed algorithm, a systematic analysis of the simulation runtime for 
the MV model was conducted on various parallel computing devices (GeForce RTX4090, Tesla P100, NVIDIA V100, and Xeon $5115\times2$ CPUs), 
with the corresponding data presented in Table \ref{tab::mitral_valve::model::parallel}. 
Similarly, the speedup ratio is defined as the runtime on each device relative to that of the 20-core CPU 
implementation using the IBAMR framework described in \cite{griffith2017hybrid}.
The results indicate that the proposed IB algorithm demonstrates outstanding computational performance 
on GPU platforms: the simulation on the RTX4090 
achieves a speedup of $57.4\times$ compared to the 20-core CPU, while the P100 and V100 achieve speedups of $28.96\times$ and $35.24\times$, 
respectively, clearly highlighting the efficiency of the proposed method on various GPU devices. 
Furthermore, a detailed comparison of the runtime distribution across major algorithm modules was performed on different GPU devices, 
as illustrated in Fig.\,\ref{fig::mitral_valve::model::percentage}. 
The analysis indicates that solving the Poisson equation remains the most time-consuming component of the computation, 
consistently accounting for over $47\%$ of the total runtime across all GPU devices. 
The solver for structural force also contributes more than $15\%$ of the total computational cost. 
Compared with the AV model, 
this increased cost is likely due to the denser solid mesh, more complex geometry
% , and the inherent nonlinearity and computational demands 
of the solid mechanics model. In contrast, with the support of GPU acceleration, the execution times of the remaining functional 
modules are significantly reduced, each accounting for less than $10\%$ of the total runtime. These findings further demonstrate the 
effectiveness of the proposed algorithm in enhancing overall computational performance.



==> chp_numerical_discretization_CG.tex <==
 
\section{Numerical Discretization}\label{sec::numerical_discretization}

% \subsection{Temporal discretization}
% We begin by considering the temporal semi-discretization for system \eqref{IB::continuous::equations}. The time interval 
% $[0,T]$ is partitioned into $N$ uniformly spaced, non-overlapping subintervals $(t_{n}, t_{n+1}]$, where $n=1,2,...,N$, 
% with a constant time step size $t_{n+1}-t_{n}=\Delta t$. Here, $(\cdot)^{n}$ denotes the value of $(\cdot)$ at time $t_{n}$.
% In this work, the modified backward Euler time-stepping scheme is employed for the temporal discretization \cite{ma2024unconditionally}, 
% and the resulting semi-discrete system is given as follows:

% \begin{subequations}\label{Equation:temporal discretization}
%     \begin{equation}
%         \frac{\rho}{\Delta t}D_h^{SL}\mathbf{u}^{n+1}=\mu\Delta\mathbf{u}^{n+1}-\nabla p^{n+1}+\mathbf{f}^{n},\label{Equation:temporal discretization::1}\\
%     \end{equation}
%     \begin{equation}
%         \nabla\cdot\mathbf{u}^{n+1}=0,                                                                                                                            \label{Equation:temporal discretization::2}\\
%     \end{equation}
%     \begin{equation}
%         \int_{B_{r}}\mathbf{F}^{n}\cdot \mathbf{V}(\mathbf{X})d\mathbf{X}=-\int_{B_{r}}\mathbb{P}^{n}:\nabla_{\mathbf{X}}\mathbf{V}(\mathbf{X})d\mathbf{X},      \label{Equation:temporal discretization::solid_force}\\
%     \end{equation}
%     \begin{equation}
%         \mathbf{f}^{n}=\mathcal{E}(\mathcal{X}^{n},\mathbf{F}^{n}),                                                                                              \label{Equation:temporal discretization::force}\\
%     \end{equation}
%     \begin{equation}
%         \mathcal{X}^{n+1}=\mathcal{X}^{n}+\Delta t \;\mathcal{I}(\mathcal{X}^{n},\mathbf{u}^{n}).                                                             \label{Equation:temporal discretization::velocity}
%     \end{equation}
% \end{subequations}
% Here, \( D_h^{SL} \mathbf{u}^{n+1} = \mathbf{u}\left(\mathbf{x}(t_{n+1}), t_{n+1}\right) - \mathbf{u}\left(\mathbf{x}(t_n), t_n\right) \) 
% represents the first-order semi-Lagrangian discretization, derived from the material derivative \(\frac{D}{Dt}\). 
% This approach eliminates the need to discretize the advection term, as detailed in \cite{phillips2001semi}.
% \eqrefs{Equation:temporal discretization} employs an explicit scheme for the FSI problems, 
% where the force term \(\mathbf{f}^n\) depends only on quantities at time \(t_n\). 
% Although implicit schemes allow larger time steps \cite{newren2007unconditionally,le2009implicit}, 
% their implementation on GPUs is challenging due to the need to solve large, nonlinear systems. 
% Thus, explicit schemes are preferred for their simplicity and computational efficiency in large-scale numerical simulations.

% \subsection{Spatial discretization}

% In the spatial discretization, we adopt the staggered-grid Marker-and-Cell (MAC) approach for the Eulerian domain, 
% following the approach of \cite{griffith2017hybrid, wells2023nodal}, 
% to approximate the Eulerian variables defined in the incompressible Navier-Stokes equations.
% Taking the three-dimensional space as an example, the computational domain $\Omega$ is discretized into uniform grid cells, 
% where the cell length in each coordinate direction ($x$, $y$, $z$) is $h$, forming a structured grid system. 
% Eulerian variables, including pressure $p$, velocity $\mathbf{u}=(u^{1},u^{2},u^{3})$, and force $\mathbf{f}=(f^{1},f^{2},f^{3})$, 
% are defined on a staggered grid, as shown in Fig.\,\ref{fig::spatial_discretization::navier_stokes}. Specifically, the pressure $p$ is located at the cell center, 
% while the velocity components $u^{1}$, $u^{2}$, and $u^{3}$ are positioned at the centers of the cell faces perpendicular to 
% the $x$, $y$, and $z$ axes, respectively. The force components $f^{1}$, $f^{2}$, and $f^{3}$ are collocated with the corresponding 
% velocity components. 
% By spatially offsetting pressure and velocity components, the staggered grid arrangement is employed to prevent the checkerboard instability.

% % \begin{figure}[!ht]
% %     \centering
% %     \begin{subfigure}[b]{0.45\textwidth}
% %         \centering
% %         \includegraphics[height=0.6\textwidth]{figure/staggered_grid.png}
% %         \caption{\label{fig::spatial_discretization::navier_stokes}}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.45\textwidth}
% %         \centering
% %         \includegraphics[height=0.6\textwidth]{figure/Xnip2025-04-02_16-33-53.jpg}
% %         \caption{\label{fig::spatial_discretization::structure}}
% %     \end{subfigure}
% %     \caption{
% %         (a) Schematic diagram of the staggered grid arrangement of Eulerian 
% %         variables in the xy-plane within a three-dimensional space. 
% %         (b) Coordinates associated with degrees of freedom of the 
% %         unstructured tetrahedron.}
% % \end{figure}
% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.4\textwidth]{figure/staggered_grid.jpg}
%     \caption{
%         Schematic of the staggered grid arrangement for Eulerian variables in the xy-plane, embedded in a three-dimensional computational domain. 
%         The red lines represents the boundaries of the computational domain, outside of which are ghost cells.
%         \label{fig::spatial_discretization::navier_stokes}
%         }
% \end{figure}
% For the Lagrangian domain, let $\mathcal{T}_h$ be a consistent triangulation of $B_{r}$ in a finite number $(N)$ of simplices.
% Define $M$ nodes on $\mathcal{T}_h$ for FE basis, and define a $3M$-dimensional vector-valued approximation space as $\mathcal{V}_h$.
% Notably, $M$ is larger than mesh nodes as shown in Fig.\,\ref{fig::algorithm:solid_GPU}.
% Let $\{\mathbf{\phi}_{l}\}$ be the standard nodally interpolating 
% finite element basis of $\mathcal{V}^{h}$. Consequently, for each node there are exactly 
% three basis functions that are nonzero at that node. For example, $k$, $M+k$, and $2M+k$ are the unique indices such that
% \begin{align*}
%     \mathbf{\phi}_{k}(\mathbf{X}_{k})=(1,0,0), \quad \mathbf{\phi}_{M+k}(\mathbf{X}_{k})=(0,1,0),\quad \mathbf{\phi}_{2M+k}(\mathbf{X}_{k})=(0,0,1),
% \end{align*}
% and otherwise $\mathbf{\phi}_{i}(\mathbf{X}_{k})=(0,0,0)$ for $i\neq k$, $i\neq M+k$, and $i\neq 2M+k$.

% The deformation $\mathcal{X}$, velocity $\mathbf{U}$, and force $\mathbf{F}$ fields are all approximated in $\mathcal{V}^{h}$.
% For convenience of notation, we ignore the explicit dependence on time  $t$ in $\mathcal{X}$, $\mathbf{U}$ and $\mathbf{F}$. 
% These quantities can be written as:
% \begin{align*}
%     &\mathcal{X}_{h}(\mathbf{X})=\sum_{l=1}^{3M}\mathcal{X}_{l}\mathbf{\phi}_{l}(\mathbf{X}),\\
%     &\mathbf{U}_{h}(\mathbf{X})=\sum_{l=1}^{3M}U_{l}\mathbf{\phi}_{l}(\mathbf{X}),\quad\\
%     &\mathbf{F}_{h}(\mathbf{X})=\sum_{l=1}^{3M}F_{l}\mathbf{\phi}_{l}(\mathbf{X}),
% \end{align*}
% where $\mathbf{\phi}_l(\mathbf{X})$ are the basis functions and $\mathcal{X}_l$, $U_l$, and $F_l$ are the corresponding coefficients.

% \subsection{Discretization for Eulerian-Lagrangian coupling operators}







% % This subsection focuses on the discretization of \eqref{Equation:temporal discretization::solid_force},  
% % \eqref{Equation:temporal discretization::force}, and \eqref{Equation:temporal discretization::velocity}.  
% % We adopt the IB-4 regularized delta function $\delta_{h}$ proposed by Peskin \cite{peskin2002immersed}.

% % Following the notation in \cite{wells2023nodal}, we apply both the **nodal quadrature rule** and the **higher-order quadrature rule**.  
% % The force term $\mathbf{F}(\mathbf{X}_q)$ is evaluated using the degrees of freedom associated with the finite element basis functions $\phi_q(\mathbf{X})$.


% This subsection focuses on the discretization of \eqref{Equation:temporal discretization::solid_force}, 
% \eqref{Equation:temporal discretization::force} and \eqref{Equation:temporal discretization::velocity}. 
% We adopt the IB-4 regularized delta function $\delta_{h}$ proposed by Peskin \cite{peskin2002immersed}.
% Following the notation in \cite{wells2023nodal}, We apply both the nodal quadrature rule and the 
% higher-order quadrature rule.
% % $\mathbf{F}(\mathbf{\mathbf{X}_q})$ can be evaluated as the freedom of the finite element basis function $\phi_{q}(\mathbf{X})$.
% \begin{itemize}
%     \item The nodal quadrature rule is defined as
%     \begin{align}
%         \mathbb{N}_{q}=\{(\mathbf{X}_{q},w_{q})\}^{M}_{q=1}, \label{Discrete::nodal_quadrature_rule}
%     \end{align}
%     where $\phi_{q}(\mathbf{X})$ is the basis function associated with node $\mathbf{X}_q$,
%     $w_{q}=\int\phi_{q}(\mathbf{X})\cdot \mathbf{1} \DX$ is 
%     the integration weight and 10 nodes are associated with every tetrahedron,
%     as in Fig.\,\ref{fig::algorithm:solid_GPU}. 
%     The approximation
%     of the left-hand part of \eqref{Equation:temporal discretization::solid_force} is approximated as:
%     \begin{equation}
%         \sum_{(\mathbf{X}_q,w_q)\in\mathbb{N}_q}\mathbf{F}_h(\mathbf{X}_q)\cdot\phi_l(\mathbf{X}_q)w_q\approx\int_{B_r} \mathbf{F} \cdot \phi_l(\mathbf{X}) d \mathbf{X},  \quad \forall \mathbf{\phi}_{l}\in\mathcal{V}^{h}.
%     \end{equation}
%     \item The higher-order quadrature rule is defined as:
%     \begin{align}
%         \mathbb{H}_{q}=\{(\mathbf{X}_{q},w_{q})\}^{M'}_{q=1}, \label{Discrete::higher_order_quadrature_rule}
%     \end{align}
%     where  $M'$ depends on the complexity of constitutive law. In this work, we adopt a 7th-order Gauss quadrature rule, and 64 quadrature nodes
%     are inside each tetrahedron. The right-hand side of \eqref{Equation:temporal discretization::solid_force} is approximation by:
%     \begin{align}
%         -\sum_{(\mathbf{X}_{q},w_{q})\in\mathbb{H}_{q}}\mathbb{P}^{e}\left(\mathcal{X}_h(\mathbf{X}_{q})\right):\nabla_{\mathbf{X}}\mathbf{\phi}_{l}(\mathbf{X}_{q})w_{q}\approx
%         -\int_{B_{r}}\mathbb{P}^{e}(\mathbf{X},t):\nabla_{\mathbf{X}}\mathbf{\phi}_{l}(\mathbf{X})d\mathbf{X}, \quad \forall \mathbf{\phi}_{l}\in\mathcal{V}^{h}.
%     \end{align}
% \end{itemize}
% As shown in the nodal scheme \cite{wells2023nodal}, neither \( F_l \) nor the weights \( w_q \) from \( \mathbb{N}_q \) need to be computed explicitly during the assembly 
% or force spreading steps. Instead, we assemble the right-hand side of \eqref{Equation:temporal discretization::solid_force} using a higher-order quadrature rule. 
% The resulting quantity, denoted \( \hat{F}_l \), represents the contribution of the basis function \( \phi_l \), given by:
% \begin{align}\label{equation::discrete::force}
%     \hat{F}_{l}=-\sum_{(\mathbf{X}_{q},w_{q})\in\mathbb{H}_{q}}\mathbb{P}^{e}\left(\mathcal{X}_h(\mathbf{X}_{q})\right):\nabla_{\mathbf{X}}\phi_{l}(\mathbf{X}_{q})w_{q}.
% \end{align}
% Then, $\hat{F}_l$ is transferred from the Lagrangian mesh to the Cartesian grid using the regularized delta function $\delta_h$, 
% based on the corresponding node on current configuration $\mathcal{X}_h(\mathbf{X}_l)$, as follows:
% \begin{align}\label{equation::discrete::force::nodal}
%     &f^{1}_{i+\frac{1}{2},j,k}=\sum_{l=1}^M\hat{F}_{l}\delta_{h}(\mathbf{x}_{i+\frac{1}{2},j,k}-\mathcal{X}_{h}(\mathbf{X}_{l})),\nonumber\\
%     &f^{2}_{i,j+\frac{1}{2},k}=\sum_{l=1}^M\hat{F}_{M+l}\delta_{h}(\mathbf{x}_{i,j+\frac{1}{2},k}-\mathcal{X}_{h}(\mathbf{X}_{l})),\nonumber\\
%     &f^{3}_{i,j,k+\frac{1}{2}}=\sum_{l=1}^M\hat{F}_{2M+l}\delta_{h}(\mathbf{x}_{i,j,k+\frac{1}{2}}-\mathcal{X}_{h}(\mathbf{X}_{l})).
% \end{align}
% Here, $M$ is the number of basis defined above. 
% The Eulerian velocity $\mathbf{u}^{n}_{h}$ is interpolated from the Cartesian grid to the structural mesh similarly as follows:
% \begin{align}\label{equation::discrete::velocity::nodal}
%     U_{l} &= \sum_{i,j,k} u^{1}_{i+\frac{1}{2},j,k} \delta_{h}(\mathbf{x}_{i+\frac{1}{2},j,k} - \mathcal{X}_{h}(\mathbf{X}_{l})) h^{3}, \nonumber \\
%     U_{M+l} &= \sum_{i,j,k} u^{2}_{i,j+\frac{1}{2},k} \delta_{h}(\mathbf{x}_{i,j+\frac{1}{2},k} - \mathcal{X}_{h}(\mathbf{X}_{l})) h^{3}, \nonumber \\
%     U_{2M+l} &= \sum_{i,j,k} u^{3}_{i,j,k+\frac{1}{2}} \delta_{h}(\mathbf{x}_{i,j,k+\frac{1}{2}} - \mathcal{X}_{h}(\mathbf{X}_{l})) h^{3}.
% \end{align}
% The duality and accuracy of the discretization scheme are further discussed in \cite{wells2023nodal}. 
% \section{Fully GPU-accelerated matrix-free algorithm}\label{sec::implementation}
% We begin by discussing the computational methods used for the fluid and solid solvers on the GPU, followed by the complete FSI algorithm. 
% All components are implemented in a matrix-free manner to ensure high computational efficiency.

% \subsection{Solver for Navier-Stokes equations}
% In the numerical solution of \eqref{Equation:temporal discretization::1} and \eqref{Equation:temporal discretization::2}, 
% we first decompose the equations using Chorin's projection method and the semi-Lagrangian method, as shown below:
% \begin{align}
%     \frac{\rho}{\Delta t}\left(\hat{\hat{\mathbf{u}}}_{h}-\hat{\mathbf{u}}_{h}^{n}\right)-\mu\Delta_{h}\hat{\hat{\mathbf{u}}}_{h}=\mathbf{f}^{n},\label{Equation:solver:NS::2}\\
%     \Delta_{h}p_{h}^{n+1}=\frac{1}{\Delta t}\nabla_{h}\cdot\hat{\hat{\mathbf{u}}}_{h},\label{Equation:solver:NS::3}\\
%     \mathbf{u}_{h}^{n+1}=\hat{\hat{\mathbf{u}}}_{h}-\Delta t\nabla_{h} p_{h}^{n+1}.\label{Equation:solver:NS::4}
% \end{align}
% Here, $\hat{\mathbf{u}}_{h}^n$ is calculated using a semi-Lagrangian approach:
% \begin{equation}\label{Equation:solver:NS::1}
%     \hat{\mathbf{u}}_{h}(\mathbf{x},t_n)=\mathbf{u}_{h}\left(\mathbf{x}-\Delta t\;\mathbf{u}_{h}^n,t_n\right).
% \end{equation}
% and \eqref{Equation:solver:NS::2} corresponds to a Helmholtz equation.
% The pressure correction in \eqref{Equation:solver:NS::3} is formulated as a Poisson equation,
% and \eqref{Equation:solver:NS::4} completes the velocity update.

% % To address boundary condition issues and avoid warp divergence on the GPU,
% % we express the original variable as $u = u' + u''$, where $u'$ is a constructed function satisfying the boundary conditions.
% % Substituting $u = u' + u''$ into the original equations yields an equation for $u''$,
% % which satisfies homogeneous Neumann or Dirichlet boundary conditions, thereby simplifying the numerical treatment of boundaries.

% The Eulerian velocity from the previous time step is first interpolated onto the staggered grid nodes.  
% Backward characteristic tracing is then performed, and the velocity at the traced-back positions is 
% interpolated using a texture memory wrapper, yielding $\hat{\mathbf{u}}_h^n$ via the semi-Lagrangian method.  
% Next, we solve the Helmholtz equation \eqref{Equation:solver:NS::2} using a matrix-free red-black Gauss-Seidel 
% iteration, where the red-black ordering ensures consistent results under parallel computation.  
% This process produces the tentative velocity $\hat{\hat{\mathbf{u}}}_h^n$.  
% In our method, since the time step is sufficiently small and the initial guess is close to the 
% solution, the red-black Gauss-Seidel iteration converges rapidly for the Helmholtz problem.  
% However, for the Poisson equation \eqref{Equation:solver:NS::3}, direct use of the 
% red-black Gauss-Seidel iteration converges extremely slowly.  
% To address this, we employ a geometric multigrid method, with the red-black Gauss-Seidel 
% iteration serving as the smoother, also in a matrix-free way.  
% Trilinear interpolation and full-weighting operators are used for prolongation and restriction, respectively.  
% We adopt a V-cycle strategy, where the residual is reduced to a prescribed threshold 
% within just a few V-cycles, yielding the pressure field $p_h^{n+1}$.  
% Finally, velocity correction is applied based on \eqref{Equation:solver:NS::3} to obtain the updated velocity $\mathbf{u}_h^{n+1}$.

% Our Navier-Stokes solver differs from the approach used in \cite{wells2023nodal}, 
% where a Crank-Nicolson (CN) scheme is used and the piecewise parabolic method (PPM) 
% were employed to discretize the convective terms. In contrast, our method 
% is designed with a greater emphasis on computational efficiency.

% \subsection{Solver for structural force}
% % To efficiently compute the structural forces in Eq.,\eqref{equation::discrete::force}, we 
% % 将基函数相关的信息存储在
% % constant memory as in Fig.\,\ref{fig::algorithm:solid_GPU}, which enables single-cycle broadcast of read-only data to all threads within a block. 
% % During initialization, the values and derivatives of the basis functions at quadrature points are 
% % precomputed and stored in constant memory. This allocation requires  
% % $(1 + 3) \times 64 \times 10 \times 8\,\text{B} = 20\,\text{KB}$,  
% % accounting for function values and gradients (1 + 3), 64 quadrature points, 10 basis functions, 
% % and double-precision storage. This setup supports 7th-order quadrature accuracy. Additionally, 
% % constitutive material parameters are also loaded into constant memory, keeping total usage well 
% % within the 64KB limit.

% To efficiently compute the structural forces in \eqref{equation::discrete::force}, we 
% store the basis function data in constant memory as shown in Fig.\,\ref{fig::algorithm:solid_GPU}. 
% This allows for single-cycle broadcasting of read-only data to all threads within a block. During 
% initialization, the values and derivatives of the basis functions at quadrature points are precomputed 
% and stored. This allocation requires $(1 + 3) \times 64 \times 10 \times 8\,\text{B} = 20\,\text{KB}$, 
% which accounts (1 + 3) values for basis functions and their derivatives, 64 quadrature points, 10 basis functions, 
% and double-precision storage. This setup ensures 7th-order quadrature accuracy. Additionally, 
% the constitutive material parameters are also loaded into constant memory, keeping the total memory 
% usage well within the $64\,\text{KB}$ limit.

% Element data, as shown in Fig.\,\ref{fig::algorithm:solid_GPU}, is precomputed and stored in global memory. 
% During preprocessing, we compute and store the following:
% 1. The inverse of the Jacobian matrix for each element, which maps points on local element to the reference element;
% 2. The volume of each element;
% 3. The map of DoFs, which is 10 integer values per element.
% For fiber-reinforced materials, fiber and sheet directions are also stored per element. Altogether, the memory required per element is approximately:  
% \((3 \times 3 + 1 + 3 + 3) \times 8\,\text{B} + 10 \times 4\,\text{B} = 168\,\text{B}\).  
% While this increases memory usage, it significantly improves runtime performance by avoiding redundant computations during the simulation.

% Furthermore, the current configuration \({\mathcal{X}}_h(t)\), 
% the initial configuration \({\mathcal{X}}_h(0)\) (used for tethering), 
% and the resulting structural forces \(\hat{\mathbf{F}}_h(t)\) are all stored in global 
% vectors as the coefficients of the basis functions, as shown in Fig.\,\ref{fig::algorithm:solid_GPU}. 
% These coefficients define the functions within the finite element space and can be efficiently 
% accessed using the precompute map for DoFs.

% For the forces applied on the structural boundaries, we follow the same methodology as for the volumetric 
% forces, with the quadrature points specifically defined on the boundary surfaces.


% % During the initialization, the values and derivatives of basis functions on quadrature points 
% % are precomputed and stored in constant memory. This allocation uses 
% % (1+3)×64×10×8B=20KB of constant memory, with 64 quadrature points, 10 basis functions, and double precision,
% % providing 7th order of quadrature accuracy. 
% % Constitutive parameters are also loaded into constant memory. 
% % These values are well within the GPU's 64KB constant memory limit.

% % During the preprocessing stage, we precompute the inverse of the Jacobian matrix for each solid element, which is used to . Additionally, we calculate and store the volume of each element in advance. While traversing all solid elements, we also record the degree-of-freedom mapping (dofmap), with each element associated with 10 integer degrees of freedom.
% % Given that the material is fiber-reinforced, the fiber and sheet directions are also stored for each element. To store all of this information—including the inverse Jacobian matrix, element volume, degree-of-freedom mapping, and fiber and sheet directions—in the global memory of the GPU, each element requires approximately:
% % (3×3+1+3+3)×8B+10×4B=168B(3 \times 3 + 1 + 3 + 3) \times 8\, \text{B} + 10 \times 4\, \text{B} = 168\, \text{B}(3×3+1+3+3)×8B+10×4B=168B Although this approach increases memory usage, it significantly improves computational efficiency by avoiding redundant calculations during the simulation process.

% % Additionally, we precompute the inverse of the Jacobian matrix for each element, 
% % which maps points from the local element to the the reference element.  we precompute as well as the local element volume. 
% % We also iterate over the elements to store the degree-of-freedom map (dofmap) for every element, 
% % which is 10 integral values per element.
% % Considering the sheet and fiber directions in fiber-reinforced materials, the memory footprint per element is approximately
% % (3×3+1+3+3)×8B+10×4B=168B. While our strategy increases memory consumption, it significantly accelerates computation.

% % The displacements $\hat{\mathcal{X}}_h(t)$, the initial positions $\hat{\mathcal{X}}_h(0)$ (for tethering), along with 
% % the resulting structural forces $\hat{\mathbf{F}}_h(t)$ 
% % of the structure, are stored in a global vector as coefficients of the basis functions.
% % % effectively forming a function within the finite element space. 
% % The coefficients associated with each element are accessible via the degree-of-freedom map (dofmap).

% % In addition, the displacement X^h(t)\hat{X}_h(t)X^h(t), the initial configuration X^h(0)\hat{X}_h(0)X^h(0) (used for anchoring), and the resulting structural force F^h(t)\hat{F}_h(t)F^h(t) are stored in a global vector as coefficients of the basis functions. The coefficients corresponding to each element can be efficiently accessed via the previously constructed degree-of-freedom mapping (dofmap).






% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.9\textwidth]{figure/solid_GPU.png}
%     \caption{
%         Efficient memory management for structural force computation
%         \label{fig::algorithm:solid_GPU}
%     }
% \end{figure}

% Based on the memory management described above, we now turn to the calculation process.
% In our implementation, the force vector assembly is carefully optimized. For each element, 
% we begin by gathering information of the map of DoFs, fiber direction, sheet direction, the inverse Jacobian, and the element volume. 
% After reading the the map of DoFs, we retrieve the current configuration, initial configuration, and reset the structural force accumulator. 
% Then, data about basis functions is broadcasted from constant memory to all threads in the block.
% Structural forces are then computed per element and written back to the global vector according to the map of DoFs. 
% To ensure the safe accumulation of contributions into the global force vector, atomic operations are used, 
% preventing race conditions during parallel writes \cite{guide2020cuda}.

% % \begin{table}[H]
% %     \centering
% %     \begin{tabular}{cccccc}
% %     \toprule
% %     \multirow{2}{*}{\textbf{Models}} && \multicolumn{4}{c}{Number of Elements} \\
% %     \cmidrule(lr){3-6}
% %      && 6000 & 48000 & 384000 & 3072000 \\
% %      \midrule
% %      \multirow{3}{*}{\textbf{SFRH}}  & GPU & 1.93 & 3.32 & 16.45 & 124.48 \\
% %                                      & CPU & 34.20 & 251.62 & 2019.24 & 16395.80 \\
% %                                      & speedup & 17.73 & 75.77 & 122.84 & 131.72 \\
% %     \midrule
% %     \multirow{3}{*}{\textbf{FHR1}}  & GPU & 2.01 & 3.61 & 19.76 & 150.08 \\
% %                                     & CPU & 48.45 & 365.05 & 2952.43 & 23617.87  \\
% %                                     & speedup & 24.15 & 101.12 & 149.39 & 157.37  \\
% %     \midrule
% %     \multirow{3}{*}{\textbf{FHR2}}  & GPU & 2.23 & 3.97 & 21.77 & 165.65 \\
% %                                     & CPU & 55.67 & 420.08 & 3464.07 & 27206.80 \\
% %                                     & speedup & 24.98 & 105.79 & 159.12 & 164.24 \\
% %     \midrule
% %     \multirow{3}{*}{\textbf{HO}}    & GPU & 2.93 & 5.45 & 30.42 & 229.53 \\
% %                                     & CPU & 69.23 &	530.84 & 4261.60 & 34124.16 \\ 
% %                                     & speedup & 23.62 & 97.46  & 140.08  & 148.67  \\
% %     \bottomrule
% %     \end{tabular}
% %     \caption{Times cost (in microseconds) for the structural solver on CPU and GPU for different kind of constitutive models and different number of elements.}
% %     \label{tab::structural::solver::performance}
% % \end{table}

% \begin{table}[H]
%     \centering
%     \begin{tabular}{cccccc}
%     \toprule
%     \multirow{2}{*}{\textbf{Model}} && \multicolumn{4}{c}{\textbf{Number of Elements}} \\
%     \cmidrule(lr){3-6}
%      && 6000 & 48000 & 384000 & 3072000 \\
%      \midrule
%      \multirow{3}{*}{\textbf{SFRH}}  & GPU & 1.93 & 3.32 & 16.45 & 124.48 \\
%                                      & CPU & 34.20 & 251.62 & 2019.24 & 16395.80 \\
%                                      & speedup & 17.73 & 75.77 & 122.84 & 131.72 \\
%     \midrule
%     \multirow{3}{*}{\textbf{FHR1}}  & GPU & 2.01 & 3.61 & 19.76 & 150.08 \\
%                                     & CPU & 48.45 & 365.05 & 2952.43 & 23617.87  \\
%                                     & speedup & 24.15 & 101.12 & 149.39 & 157.37  \\
%     \midrule
%     \multirow{3}{*}{\textbf{FHR2}}  & GPU & 2.23 & 3.97 & 21.77 & 165.65 \\
%                                     & CPU & 55.67 & 420.08 & 3464.07 & 27206.80 \\
%                                     & speedup & 24.98 & 105.79 & 159.12 & 164.24 \\
%     \midrule
%     \multirow{3}{*}{\textbf{HO}}    & GPU & 2.93 & 5.45 & 30.42 & 229.53 \\
%                                     & CPU & 69.23 & 530.84 & 4261.60 & 34124.16 \\ 
%                                     & speedup & 23.62 & 97.46  & 140.08  & 148.67  \\
%     \bottomrule
%     \end{tabular}
%     \caption{Execution time (in milliseconds) of the structural solver for various constitutive models and mesh sizes on both CPU and GPU platforms.}
%     \label{tab::structural::solver::performance}
% \end{table}


% Table~\ref{tab::structural::solver::performance} presents the execution time and speedup 
% of the structural solver on both a single-core CPU and a GPU, across a variety of constitutive models 
% and varying numbers of elements. Despite the solver's reliance on double-precision floating-point operations 
% and irregular memory access patterns, our GPU implementation achieves up to approximately $150\times$ speedup 
% in large-scale simulations. All constitutive models achieve ideal speedup, 
% though their execution times vary primarily due to differences in computational complexity, 
% such as the presence of nonlinear functions or intricate tensor operations.

% \subsection{Fluid-structure coupling}

% % \textcolor{black}{
% % The coupling between Eulerian and Lagrangian variables is achieved through the discretization 
% % of the interpolation and spreading operators. }
% % 计算中，耦合流体求解器和固体求解器通过计算的插值算子和延拓算子
% % The continuous form of the equations are given 
% % by \eqref{eq::IB::continuous::spreading} and \eqref{eq::IB::continuous::interpolation}, while 
% In the computational framework of IB method, 
% the solvers for Navier-Stokes equations and structural force are coupled 
% through discrete interpolation and spreading operators 
% given by \eqref{equation::discrete::velocity::nodal} 
% and \eqref{equation::discrete::force::nodal}, and their practical implementations are 
% illustrated in \figref{fig::ELI}a and \figref{fig::ELI}b.
% % Unlike the calculation of structural forces, where each element is assigned a 
% % single thread, 
% For both operators, each Lagrangian node is assigned one thread, and the number of total threads is $M$. 
% It allows maintaining a complexity of $O(M)$ because each Lagrangian 
% node can directly compute the indices of the neighboring Eulerian grid cells without 
% needing to traverse all grid cells. 
% For the force spreading algorithm, based on the current configuration 
% of each Lagrangian node, we first calculate the index of the corresponding Eulerian grid cell. 
% Then, depending on the choice of the regularized delta function $\delta_h$, 
% the neighboring grid cells are identified. The contributions of the Eulerian forces
% are subsequently calculated and spread to the adjacent Eulerian 
% grid cells using atomic operations.
% For the velocity interpolation algorithm, the velocity from the Eulerian grid 
% are interpolated to the Lagrangian nodes. After identifying the neighboring grid cells, 
% the threads read the velocity data and calculate the corresponding Lagrangian node values. 
% Finally, the current configuration of Lagrangian nodes is updated.


% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.9\textwidth]{figure/ELI-spreading.png}
%     \caption{\label{fig::ELI}
%         (a) GPU-based force spreading algorithm: Illustration of the process for transferring Lagrangian structural forces to the Eulerian grid using atomic operations, based on the current structural configuration.
%         (b) GPU-based velocity interpolation and configuration update: Illustration of the process for interpolating Eulerian velocity to Lagrangian nodes and updating the structural configuration accordingly.}
% \end{figure}

% The complete FSI algorithm at each time step is illustrated in \figref{fig:algorithm:total}. 
% Our implementation employs an explicit coupling scheme with a staggered approach, 
% which enables decoupled solving of the fluid and solid subsystems.
% The key coupling procedure consists of the following stages:
% \begin{enumerate}
%     \item \textbf{Structural Force Solver.} Solve the structural force in the Lagrangian mesh:
%     $\mathcal{X}_h^{n} \rightarrow \hat{\mathbf{F}}_h^{n}$;
%     \item \textbf{Lagrangian to Eulerian.} Spread the structural force onto the Eulerian grid:
%     $\hat{\mathbf{F}}_h^{n} \rightarrow \mathbf{f}_h^{n}$;
%     \item \textbf{Navier-Stokes Solver.} Solve the velocity in the Eulerian grid:
%     $\{\mathbf{u}_h^{n},\mathbf{f}_h^{n}\}\rightarrow\mathbf{u}_h^{n+1}$;
%     \item \textbf{Eulerian to Lagrangian.} Interpolate the velocity into the Lagrangian mesh and update its current configuration:
%     $\mathbf{u}^{n+1} \rightarrow \mathcal{X}_h^{n+1}$.
% \end{enumerate}

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figure/algorithm-total.png}
%     \caption{
%         Schematic graph for the fully GPU-accelerated matrix-free algorithm for FSI within a timestep.
%         % Setup of the anisotropic Cook's membrane benchmark: The gray region represents the fixed computational domain $\Omega$, while the red region corresponds to the deformable structure.
%         \label{fig:algorithm:total}
%         }
% \end{figure}
% In summary, the algorithm utilizes GPU optimizations, 
% including texture memory, constant memory for basis functions, and 
% efficient iterative solvers like red-black Gauss-Seidel with
% multigrid acceleration. These techniques together create a 
% robust and efficient fluid-structure coupling framework.
% % \subsection{Computational devices}
% We perform simulations primarily on a GeForce RTX 4090 GPU, 
% with additional tests on NVIDIA V100 and P100 GPUs for comparison. 
% CPU-based simulations using IBAMR of version 0.5.1 run on a dual 
% Intel Xeon 5115 workstation (10 cores per CPU).
% Notably, the RTX 4090 is a consumer-grade GPU with limited 
% double-precision performance (1/64 of single-precision) 
% and restricted multi-GPU capabilities, but at a fraction 
% of the cost of professional cards, making it highly 
% suitable for practical applications.
% Our results show the RTX 4090 is fully adequate for our simulations, 
% and we expect future GPU advances to further improve our 
% framework's ability to handle complex cardiac models.


==> src/_math_commands.tex <==


